Deep Matching and Validation Network -- An End-to-End Solution to Constrained Image Splicing Localization and Detection

Image splicing is a very common image manipulation technique that is sometimes used for malicious purposes. A splicing detec- tion and localization algorithm usually takes an input image and produces a binary decision indicating whether the input image has been manipulated, and also a segmentation mask that corre- sponds to the spliced region. Most existing splicing detection and localization pipelines suffer from two main shortcomings: 1) they use handcrafted features that are not robust against subsequent processing (e.g., compression), and 2) each stage of the pipeline is usually optimized independently. In this paper we extend the formulation of the underlying splicing problem to consider two input images, a query image and a potential donor image. Here the task is to estimate the probability that the donor image has been used to splice the query image, and obtain the splicing masks for both the query and donor images. We introduce a novel deep convolutional neural network architecture, called Deep Matching and Validation Network (DMVN), which simultaneously localizes and detects image splicing. The proposed approach does not depend on handcrafted features and uses raw input images to create deep learned representations. Furthermore, the DMVN is end-to-end op- timized to produce the probability estimates and the segmentation masks. Our extensive experiments demonstrate that this approach outperforms state-of-the-art splicing detection methods by a large margin in terms of both AUC score and speed.

==> NC2017v1.tex <==

\begin{figure*}[tbph]
\centering
\scriptsize
\begin{tabular}{@{}c c c c@{}}
\includegraphics[width=.24\linewidth]{88629-19e32f2b29a2b345dfd28a8ad857b3fc_x_797a0b5dd9c47a4b391f4cee60ba9354-P7_60}&
\includegraphics[width=.24\linewidth]{1_0000-c0cfa4a6a95b3762f9d966e09a0340b9_x_030d521fca99981c442e60e4b2155699-P5_10}&
\includegraphics[width=.24\linewidth]{0_9798-9883d12156ed82344d65fe19575e1d84_x_8b570c4bd216f5144774b9c0bc61bbd4-P3_38}&
\includegraphics[width=.24\linewidth]{1_0000-4bf6a60d74ecd725e3e4b0eedc7d7cc0_x_96492c250780ebababfcebc585ef1db6-P8_32}\\
(a) (PID,QID)=&(b) (PID,QID)=&(c) (PID,QID)=&(d) (PID,QID)=\\
(19e32f2b29a2b345dfd28a8ad857b3fc,&(c0cfa4a6a95b3762f9d966e09a0340b9,&
797a0b5dd9c47a4b391f4cee60ba9354)&030d521fca99981c442e60e4b2155699)\\
(9883d12156ed82344d65fe19575e1d84,&(4bf6a60d74ecd725e3e4b0eedc7d7cc0,&
8b570c4bd216f5144774b9c0bc61bbd4)&96492c250780ebababfcebc585ef1db6)\\
\end{tabular}
\caption{Predicted splicing masks the NC2017 dataset. From top to bottom, input pair, ground truth manipulation masks (see text for explanations), DMVN predicted splicing masks, and overlaid masks.}\label{fig.visNC2017}
\end{figure*}
